Cost Minimization in Multiple IaaS Clouds: A Double Auction Approach

IaaS clouds invest substantial capital in operating their data centers. Reducing the cost of resource provisioning, is their forever pursuing goal. Computing resource trading among multiple IaaS clouds provide a potential for IaaS clouds to utilize cheaper resources to fulfill their jobs, by exploiting the diversities of different clouds' workloads and operational costs. In this paper, we focus on studying the IaaS clouds' cost reduction through computing resource trading among multiple IaaS clouds. We formulate the global cost minimization problem among multiple IaaS clouds under cooperative scenario where each individual cloud's workload and cost information is known. Taking into consideration jobs with disparate lengths, a non-preemptive approximation algorithm for leftover job migration and new job scheduling is designed. Given to the selfishness of individual clouds, we further design a randomized double auction mechanism to elicit clouds' truthful bidding for buying or selling virtual machines. We evaluate our algorithms using trace-driven simulations.

==> performance.tex <==

\section{Algorithm Performance} \label{sec:performance}

%analyze the performance of algorithm based on lyapunov optimization

Let us consider the drift-plus-penalty for frame $r$.

{\small\begin{align*}
L(\mathbf{\Theta}(rT+T)) - L(\mathbf{\Theta}(rT)) + V\sum_{\tau = rT}^{rT+T-1}\sum_{j=1}^J C_j(\tau)
\end{align*}
}

We could take control policies in one frame to minimize the drift-plus-penalty for the frame. As there are no leftover jobs in data centers at the beginning of each frame, the control policies in the previous frame will not affect the control policies in the current frame.

For every frame $r$, minimize the following frame based drift-plus-penalty, the details for the derivation of frame based drift-plus-penalty can be seen in appendix (\ref{}):

{\footnotesize\begin{align*}
\min
& \sum_{\tau=rT}^{rT+T-1} \sum_{k=1}^K \{ V [\sum_{l\in \cup\widetilde{\mathcal{U}}_j^k(\tau)\cup\mathcal{U}_j^k}c^l + \alpha^k_j G^k_j(\tau)] \\
& - [(w^k)^2q_j^k(\tau) + Z_j^k(\tau)][U_j^k(\tau) + G_j^k(\tau)] \} \\
\mbox{Constraints} & (\ref{con:dynamicQqueue}) (\ref{con:dynamicZqueue}) (\ref{con:indicator})-(\ref{placement}).
\end{align*}
} 
